Fusion rules for admissible representations of affine algebras: the case of $A_2^{(1)}$

We derive the fusion rules for a basic series of admissible representations of $\hat{sl}(3)$ at fractional level $3/p-3$. The formulae admit an interpretation in terms of the affine Weyl group introduced by Kac and Wakimoto. It replaces the ordinary affine Weyl group in the analogous formula for the fusion rules multiplicities of integrable representations. Elements of the representation theory of a hidden finite dimensional graded algebra behind the admissible representations are briefly discussed.

==> adm-pic.tex <==
%\documentclass{article}
%\usepackage{xy}
\input xy
\xyoption{all}
%\input xypic
%\input xypoly
\nopagenumbers

\def\bt{\bullet}\def\cr{\circ}\def\st{\star}\def\tm{{\rm x}}
\def\hrt{\halfrootthree}
\def\wyg{{\cal W}} \def\fwd{{\cal G}}



\bigskip

\xy 
0;<\hrt cm,.5cm>:<-\hrt cm,.5cm>::
{(-2,-2)\PATH~={**\dir{--}}'(-1,-2)'(0,-1)'(1,-1)
               '(2,0)'(3,0)'(4,1)'(5,1)'(6,2)'(7,2)
			   '(8,3)'(8,4)'(7,4)'(7,5)'(6,5)'(6,6)
			   '(5,6)'(5,7)'(4,7)'(4,8)'(3,8)'(2,7)
			   '(2,6)'(1,5)'(1,4)'(0,3)'(0,2)'(-1,1)
			   '(-1,0)'(-2,-1)'(-2,-2)},
{(0,-1)\PATH~={**\dir{--}}'(0,0)*+{00}*\frm{o}},
{(2,0)\PATH~={**\dir{--}}'(2,1)*+{21}*\frm{o}},
{(4,1)\PATH~={**\dir{--}}'(4,2)*+{01}*\frm{o}},
{(6,2)\PATH~={**\dir{--}}'(6,3)*+{30}*\frm{o}},
{(7,4)\PATH~={**\dir{--}}'(6,3)*+{30}*\frm{o}},
{(6,5)\PATH~={**\dir{--}}'(5,4)*+{02}*\frm{o}},
{(5,6)\PATH~={**\dir{--}}'(4,5)*+{20}*\frm{o}},
{(4,7)\PATH~={**\dir{--}}'(3,6)*+{03}*\frm{o}},
{(2,6)\PATH~={**\dir{--}}'(3,6)*+{03}*\frm{o}},
{(1,4)\PATH~={**\dir{--}}'(2,4)*+{10}*\frm{o}},
{(0,2)\PATH~={**\dir{--}}'(1,2)*+{12}*\frm{o}},
{(-1,0)\PATH~={**\dir{--}}'(0,0)*+{00}*\frm{o}},
%
{(-1,-1)\PATH~={**\dir{.}}'(7,3)'(3,7)'(-1,-1)},
{(-1,-1)\PATH~={**\dir{.}}'(0,-2)},
{(-1,-1)\PATH~={**\dir{.}}'(-2,-3)},
{(-1,-1)\PATH~={**\dir{.}}'(-2,0)},
{(-1,-1)\PATH~={**\dir{.}}'(-3,-2)},
{(7,3)\PATH~={**\dir{.}}'(9,4)},
{(7,3)\PATH~={**\dir{.}}'(8,2)},
{(7,3)\PATH~={**\dir{.}}'(6,1)},
{(7,3)\PATH~={**\dir{.}}'(8,5)},
{(3,7)\PATH~={**\dir{.}}'(4,9)},
{(3,7)\PATH~={**\dir{.}}'(2,8)},
{(3,7)\PATH~={**\dir{.}}'(1,6)},
{(3,7)\PATH~={**\dir{.}}'(5,8)},
%
{(0,0)*+{00}*\frm{o} \PATH ~={**\dir{-}}
                '(1,1)*+{11}*\frm{-}^0},
%
{(2,1)*+{21}*\frm{o}\PATH ~={**\dir{-}}
'(1,1)*+{11}*\frm{-}^2'(1,2)*+{12}*\frm{o}^1},
%
{(2,1)*+{21}*\frm{o}\PATH ~={**\dir{-}} '(3,2)*+{12}*\frm{-}^1},
{(1,2)*+{12}*\frm{o}\PATH ~={**\dir{-}} '(2,3)*+{21}*\frm{-}^2},
%
{(4,2)*+{01}*\frm{o}\PATH ~={**\dir{-}} '(3,2)*+{12}*\frm{-}^0
'(3,3)*+{11}*\frm{o}^2'(2,3)*+{21}*\frm{-}^1'(2,4)*+{10}*\frm{o}^0},
%
{(4,2)*+{01}*\frm{o}\PATH ~={**\dir{-}} '(5,3)*+{13}*\frm{-}^2},
{(3,3)*+{11}*\frm{o}\PATH ~={**\dir{-}} '(4,4)*+{22}*\frm{-}^0},
{(2,4)*+{10}*\frm{o}\PATH ~={**\dir{-}} '(3,5)*+{31}*\frm{-}^1},
%
{(6,3)*+{30}*\frm{o}\PATH ~={**\dir{-}} '(5,3)*+{13}*\frm{-}^1
'(5,4)*+{02}*\frm{o}^0'(4,4)*+{22}*\frm{-}^2
'(4,5)*+{20}*\frm{o}^1'(3,5)*+{31}*\frm{-}^0
'(3,6)*+{03}*\frm{o}^2},
%
\endxy
\bigskip fig. 1
\medskip%\noindent
The $p'/p=3/4$ admissible alcove.
%; the dotted lines serving as
%borders are from the dual lattice; reflecting in them gives the
%KW action; the weights $[n,m]$ are in
%circles, the weights $[[n,m]]$ in boxes
%\bye
\bigskip


\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(1,0)*+{\bt}\PATH ~={**\dir{-}}'(0,0)*+{\Lambda}*\frm{o}^1
                     '(0,1)*+{\st}^2},
%
{(1,0)*+{\bt}\PATH ~={**\dir{-}}'(2,1)*+{\bt}^2},
{(0,1)*+{\st}\PATH ~={**\dir{-}}'(1,2)*+{\cr}^1},
%
{(4,0)*+{\st}\PATH ~={**\dir{-}}'(3,0)*+{\bt}*\frm{o}^1
            '(3,1)*+{\bt}^2
            '(2,1)*+{\bt}^0'(2,2)*+{\bt}^1'(1,2)*+{\cr}^2
            '(1,3)*+{\cr}^0'(0,3)*+{\cr}*\frm{o}^1'(0,4)*+{\cr}^2},
%
{(4,0)*+{\st}\PATH ~={**\dir{-}}'(5,1)*+{\st}^2},
{(3,1)*+{\cr}\PATH ~={**\dir{-}}'(4,2)*+{\cr}^1},
{(2,2)*+{\bt}\PATH ~={**\dir{-}}'(3,3)*+{\bt}^0},
{(1,3)*+{\cr}\PATH ~={**\dir{-}}'(2,4)*+{\cr}^2},
{(0,4)*+{\cr}\PATH ~={**\dir{-}}'(1,5)*+{\cr}^1},
%
{(7,0)*+{\cr}\PATH ~={**\dir{-}}'(6,0)*+{\cr}*\frm{o}^1
            '(6,1)*+{\cr}^2
            '(5,1)*+{\st}^0'(5,2)*+{\cr}^1'(4,2)*+{\cr}^2
            '(4,3)*+{\cr}^0'(3,3)*+{\cr}*\frm{o}^1'(3,4)*+{\cr}^2
			'(2,4)*+{\cr}^0'(2,5)*+{\cr}^1'(1,5)*+{\cr}^2
		'(1,6)*+{\cr}^0'(0,6)*+{\cr}*\frm{o}^1'(0,7)*+{\cr}^2},
%
{(7,0)*+{\cr}\PATH ~={**\dir{-}}'(8,1)*+{\cr}^2},
{(6,1)*+{\cr}\PATH ~={**\dir{-}}'(7,2)*+{\cr}^1},
{(5,2)*+{\cr}\PATH ~={**\dir{-}}'(6,3)*+{\cr}^0},
{(4,3)*+{\cr}\PATH ~={**\dir{-}}'(5,4)*+{\cr}^2},
{(3,4)*+{\cr}\PATH ~={**\dir{-}}'(4,5)*+{\st}^1},
{(2,5)*+{\cr}\PATH ~={**\dir{-}}'(3,6)*+{\cr}^0},
{(1,6)*+{\cr}\PATH ~={**\dir{-}}'(2,7)*+{\cr}^2},
{(0,7)*+{\cr}\PATH ~={**\dir{-}}'(1,8)*+{\cr}^1},
%
{(10,0)*+{\cr}\PATH ~={**\dir{-}}
              '(9,0)*+{\cr}*\frm{o}^1
			  '(9,1)*+{\cr}^2'(8,1)*+{\cr}^0'(8,2)*+{\cr}^1
              '(7,2)*+{\cr}^2'(7,3)*+{\cr}^0
			  '(6,3)*+{\cr}*\frm{o}^1'(6,4)*+{\cr}^2
			  '(5,4)*+{\cr}^0'(5,5)*+{\st}^1'(4,5)*+{\st}^2
			  '(4,6)*+{\cr}^0'(3,6)*+{\cr}*\frm{o}^1
			  '(3,7)*+{\cr}^2'(2,7)*+{\cr}^0'(2,8)*+{\cr}^1
			  '(1,8)*+{\cr}^2'(1,9)*+{\cr}^0
			  '(0,9)*+{\cr}*\frm{o}^1'(0,10)*+{\cr}^2},
%
{(0,0)*+{\Lambda}\PATH ~={**\dir{=}}'(1,0)*+{\bt}'(2,1)*+{\bt}
                    '(3,1)*+{\bt}'(3,0)*+{\bt} },
{(2,1)*+{\bt}\PATH ~={**\dir{=}}'(2,2)*+{\bt}'(3,3)*+{\bt}}	
\endxy 
\bigskip fig. 2
\medskip%\noindent
The begining of $\wyg^+_\Lambda$ with
the weight diagram  $\fwd_\Lambda$, $\Lambda=[1,0]$.
%vertices of the sublattice $\Lambda+\kappa Q^+$ are placed 
%in circles; the singular vectors are indicated by stars; the
%finite diagram $\fwd_\Lambda$ cut out by the singular vectors 
%of $\Lambda=[1,0]$ is indicated by bold points and links
\bigskip\bigskip

\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(1,0)*+{\bt}\PATH ~={**\dir{-}}'(0,0)*+{\Lambda}^1'(0,1)*+{\st}^2},
%
{(1,0)*+{\bt}\PATH ~={**\dir{-}}'(2,1)*+{\bt}^2},
{(0,1)*+{\st}\PATH ~={**\dir{-}}'(1,2)*+{\cr}^1},
%
{(4,0)*+{\cr}\PATH ~={**\dir{-}}'(3,0)*+{\bt}^1'(3,1)*+{\bt}^2
            '(2,1)*+{\bt}^0'(2,2)*+{\bt}^1'(1,2)*+{\cr}^2},
%
{(4,0)*+{\cr}\PATH ~={**\dir{-}}'(5,1)*+{\cr}^2},
{(3,1)*+{\bt}\PATH ~={**\dir{-}}'(4,2)*+{\bt}^1},
{(2,2)*+{\bt}\PATH ~={**\dir{-}}'(3,3)*+{\bt}^0},
%
{(7,0)*+{\st}\PATH ~={**\dir{-}}'(6,0)*+{\bt}^1'(6,1)*+{\bt}^2
            '(5,1)*+{\cr}^0'(5,2)*+{\bt}^1'(4,2)*+{\bt}^2
            '(4,3)*+{\bt}^0'(3,3)*+{\bt}^1'(3,4)*+{\cr}^2},
%
{(7,0)*+{\st}\PATH ~={**\dir{-}}'(8,1)*+{\st}^2},
{(6,1)*+{\bt}\PATH ~={**\dir{-}}'(7,2)*+{\cr}^1},
{(5,2)*+{\bt}\PATH ~={**\dir{-}}'(6,3)*+{\bt}^0},
{(4,3)*+{\bt}\PATH ~={**\dir{-}}'(5,4)*+{\bt}^2},
{(3,4)*+{\cr}\PATH ~={**\dir{-}}'(4,5)*+{\cr}^1},
%
{(8,1)*+{\st}\PATH ~={**\dir{-}}'(8,2)*+{\cr}^1
              '(7,2)*+{\cr}^2'(7,3)*+{\cr}^0'(6,3)*+{\bt}^1
			  '(6,4)*+{\bt}^2
			  '(5,4)*+{\bt}^0'(5,5)*+{\cr}^1'(4,5)*+{\cr}^2
},
%
{(7,3)*+{\cr}\PATH ~={**\dir{-}}'(8,4)*+{\cr}^2},
{(6,4)*+{\cr}\PATH ~={**\dir{-}}'(7,5)*+{\cr}^1},
{(5,5)*+{\cr}\PATH ~={**\dir{-}}'(6,6)*+{\cr}^0},
%
{(8,4)*+{\cr}\PATH ~={**\dir{-}}
              '(8,5)*+{\cr}^1'(7,5)*+{\cr}^2'(7,6)*+{\cr}^0
			  '(6,6)*+{\cr}^1'(6,7)*+{\cr}^2},
%
{(7,6)*+{\cr}\PATH ~={**\dir{-}}'(8,7)*+{\cr}^2},
{(6,7)*+{\cr}\PATH ~={**\dir{-}}'(7,8)*+{\st}^1},
%
{(8,7)*+{\cr}\PATH ~={**\dir{-}}
              '(8,8)*+{\st}^1'(7,8)*+{\st}^2},
%
{(0,0)*+{\Lambda}*\frm{o}\PATH ~={**\dir{=}}
       '(1,0)*+{\bt}'(2,1)*+{\bt}
       '(3,1)*+{\bt}'(3,0)*+{\bt}*\frm{o} 
       '(4,0)*+{\bt}'(5,1)*+{\bt}
       '(6,1)*+{\bt}'(6,0)*+{\bt}*\frm{o}},
{(5,1)*+{\bt}\PATH ~={**\dir{=}}
       '(5,2)*+{\bt}'(6,3)*+{\bt}*\frm{o}
       '(6,4)*+{\bt}'(5,4)*+{\bt} 
	   '(5,5)*+{\bt}'(6,6)*+{\bt}*\frm{o}},	
			{(2,1)*+{\bt}\PATH ~={**\dir{=}}
       '(2,2)*+{\bt}'(3,3)*+{\bt}*\frm{o}
       '(4,3)*+{\bt}'(4,2)*+{\bt} 
	   '(3,1)*+{\bt}},
	{(4,2)*+{\bt}\PATH ~={**\dir{=}}'(5,2)*+{\bt}},	
	{(4,3)*+{\bt}\PATH ~={**\dir{=}}'(5,4)*+{\bt}}	
			
\endxy 
\bigskip fig. 3
\medskip%\noindent
The weight diagram $\fwd_{[2,0]}$. The big circles indicate the $sl(3)$
counterpart diagram $-\kappa\,\Gamma_{(2,0)}$.
% comprised of the bold vertices 
%and bold edges,
%resolved in terms of ``Verma'' modules (the singular vectors are
%indicated by stars), the points on the sublattice 
%$\Lambda+\kappa Q^+$ are in circles
\bigskip

\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
 '(0,0)*+{1}*\frm{o}^1'(0,1)*+{1}*\frm{o}^2},
%
{(1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(2,1)*+{2}*\frm{o}^2},
{(0,1)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(1,2)*+{2}*\frm{o}^1},
%
{(3,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
		 '(3,1)*+{2}*\frm{o}^2'(2,1)*+{2}*\frm{o}^0
		 '(2,2)*+{3}*\frm{o}^1'(1,2)*+{2}*\frm{o}^2
         '(1,3)*+{2}*\frm{o}^0'(0,3)*+{1}*\frm{o}^1},
%
{(3,1)*+{2}\PATH ~={**\dir{-}}'(4,2)*+{2}^1},
{(2,2)*+{3}\PATH ~={**\dir{-}}'(3,3)*+{4}^0},
{(1,3)*+{2}\PATH ~={**\dir{-}}'(2,4)*+{2}^2},
%
{(5,2)*+{1}*\frm{o}
		   \PATH ~={**\dir{-}}
		   '(4,2)*+{2}*\frm{o}^2'(4,3)*+{3}*\frm{o}^0
		   '(3,3)*+{4}*\frm{o}^1'(3,4)*+{3}*\frm{o}^2
		   '(2,4)*+{2}*\frm{o}^0'(2,5)*+{1}*\frm{o}^1},
%
{(5,2)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(6,3)*+{1}*\frm{o}^0},
{(4,3)*+{3}*\frm{o}\PATH ~={**\dir{-}}'(5,4)*+{2}*\frm{o}^2},
{(3,4)*+{3}*\frm{o}\PATH ~={**\dir{-}}'(4,5)*+{2}*\frm{o}^1},
{(2,5)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(3,6)*+{1}*\frm{o}^0},
%
{(6,3)*+{1}*\frm{o}
			  \PATH ~={**\dir{-}}
			  '(6,4)*+{1}*\frm{o}^2'(5,4)*+{2}*\frm{o}^0
			  '(5,5)*+{2}*\frm{o}^1'(4,5)*+{2}*\frm{o}^2
			  '(4,6)*+{1}*\frm{o}^0'(3,6)*+{1}*\frm{o}^1},
%
{(5,5)*+{2}\PATH ~={**\dir{-}}'(6,6)*+{1}*\frm{o}^0},
\endxy
\bigskip fig. 4 
\medskip%\noindent
The [1,1] diagram with weight multiplicities indicated in the circles.

\bigskip

\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
          '(0,0)*+{1}*\frm{o}^1'(0,1)*+{1}*\frm{o}^2},
%
{(1,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(2,1)*+{2}*\frm{o}^2},
{(0,1)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(1,2)*+{2}*\frm{o}^1},
%
{(4,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
         '(3,0)*+{1}*\frm{o}^1'(3,1)*+{2}*\frm{o}^2
         '(2,1)*+{2}*\frm{o}^0'(2,2)*+{3}*\frm{o}^1
		 '(1,2)*+{2}*\frm{o}^2'(1,3)*+{2}*\frm{o}^0
		 '(0,3)*+{1}*\frm{o}^1'(0,4)*+{1}*\frm{o}^2},
%
{(4,0)*+{1}\PATH ~={**\dir{-}}'(5,1)*+{2}^2},
{(3,1)*+{2}\PATH ~={**\dir{-}}'(4,2)*+{3}^1},
{(2,2)*+{3}\PATH ~={**\dir{-}}'(3,3)*+{4}^0},
{(1,3)*+{2}\PATH ~={**\dir{-}}'(2,4)*+{3}^2},
{(0,4)*+{1}\PATH ~={**\dir{-}}'(1,5)*+{2}^1},
%
{(6,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
           '(6,1)*+{2}*\frm{o}^2'(5,1)*+{2}*\frm{o}^0
		   '(5,2)*+{3}*\frm{o}^1'(4,2)*+{3}*\frm{o}^2
		   '(4,3)*+{4}*\frm{o}^0'(3,3)*+{4}*\frm{o}^1
		   '(3,4)*+{4}*\frm{o}^2'(2,4)*+{3}*\frm{o}^0
		   '(2,5)*+{3}*\frm{o}^1'(1,5)*+{2}*\frm{o}^2
		   '(1,6)*+{2}*\frm{o}^0'(0,6)*+{1}*\frm{o}^1},
%
{(6,0)*+{1}*\frm{o}\PATH ~={**\dir{.}}'(7,0)*+{}*\frm{}},
{(0,6)*+{1}*\frm{o}\PATH ~={**\dir{.}}'(0,7)*+{}*\frm{}},
%
{(6,1)*+{2}\PATH ~={**\dir{.}}'(7,2)*+{}*\frm{}},
{(5,2)*+{3}\PATH ~={**\dir{.}}'(6,3)*+{}*\frm{}},
{(4,3)*+{4}\PATH ~={**\dir{.}}'(5,4)*+{}*\frm{}},
{(3,4)*+{4}\PATH ~={**\dir{.}}'(4,5)*+{}*\frm{}},
{(2,5)*+{3}\PATH ~={**\dir{.}}'(3,6)*+{}*\frm{}},
{(1,6)*+{2}\PATH ~={**\dir{.}}'(2,7)*+{}*\frm{}},
%
\endxy
\bigskip fig. 5 
\medskip%\noindent
The begining of $\wyg^+$ with multiplicities indicated in circles.
\bigskip

\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
%
{(0,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(1,1)*+{2}*\frm{o}^0},
%
{(4,1)*+{2}*\frm{o}\PATH ~={**\dir{-}}
         '(3,0)*+{1}*\frm{o}^0'(2,0)*+{1}*\frm{o}^2
         '(2,1)*+{2}*\frm{o}^0'(1,1)*+{2}*\frm{o}^1
		 '(1,2)*+{2}*\frm{o}^2'(0,2)*+{1}*\frm{o}^0
		 '(0,3)*+{1}*\frm{o}^1'(1,4)*+{2}*\frm{o}^0},
%
{(2,1)*+{2}*\frm{o}\PATH ~={**\dir{-}}'(3,2)*+{3}*\frm{o}^2},
{(1,2)*+{2}*\frm{o}\PATH ~={**\dir{-}}'(2,3)*+{3}*\frm{o}^1},
%
{(5,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
         '(5,1)*+{2}*\frm{o}^0'(4,1)*+{2}*\frm{o}^1
         '(4,2)*+{3}*\frm{o}^2'(3,2)*+{3}*\frm{o}^0
		 '(3,3)*+{4}*\frm{o}^1'(2,3)*+{3}*\frm{o}^2
		 '(2,4)*+{3}*\frm{o}^0'(1,4)*+{2}*\frm{o}^1
         '(1,5)*+{2}*\frm{o}^2'(0,5)*+{1}*\frm{o}^0 },
%
{(5,0)*+{1}\PATH ~={**\dir{.}}'(6,0)*+{}},
{(0,5)*+{1}\PATH ~={**\dir{.}}'(0,6)*+{}},
\endxy
\bigskip fig. 6 
\medskip %\noindent
The beginning of $\wyg^-$ 
with multiplicities in circles.
\bigskip

\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
%
{(0,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(1,1)*+{2}*\frm{o}^0},
%
{(4,1)*+{\cr}\PATH ~={**\dir{-}}
         '(3,0)*+{\cr}^0'(2,0)*+{\st}^2
         '(2,1)*+{1}*\frm{o}^0'(1,1)*+{2}*\frm{o}^1
		 '(1,2)*+{1}*\frm{o}^2'(0,2)*+{\st}^0
		 '(0,3)*+{\cr}^1'(1,4)*+{\cr}^0},
%
{(2,1)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(3,2)*+{\cr}^2},
{(1,2)*+{1}*\frm{o}\PATH ~={**\dir{-}}'(2,3)*+{\cr}^1},
%
{(5,1)*+{\cr} \PATH ~={**\dir{-}}'(4,1)*+{\cr}^1
         '(4,2)*+{\st}^2'(3,2)*+{\cr}^0
		 '(3,3)*+{\cr}^1'(2,3)*+{\cr}^2
		 '(2,4)*+{\st}^0'(1,4)*+{\cr}
         '(1,5)*+{\cr}^2},
%
{(3,3)*+{\cr}\PATH ~={**\dir{-}}'(4,4)*+{\st}^0},
{(2,1)*+{1}*\frm{o}\PATH ~={**\dir{=}}'(1,1)*+{2}*\frm{o}
         '(1,2)*+{1}*\frm{o}},
{(0,0)*+{1}*\frm{o}\PATH ~={**\dir{=}}'(1,1)*+{2}*\frm{o}},		 
\endxy
\bigskip fig. 7 
\medskip %\noindent
The beginning of $\wyg^-$ with the resolution of [[1,1]]. 
The multiplicities of ${\cal G}_{[[1,1]]}$ are in circles.
\bigskip


\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
%0;<\hrt cm,.5cm>:<-\hrt cm,.5cm>::
{(0,0)*+{\bt}\PATH~={**\dir{.}}
               '(1,0)*+{\bt}'(2,0)*+{\bt}*\frm{-}'(3,0)*+{\bt}
               '(4,1)*+{\bt}*\frm{-}'(5,2)*+{\bt}'(6,3)*+{\bt}
			   '(7,4)*+{\bt}*\frm{-}'(8,5)*+{\bt}'(9,6)*+{\bt}
			   '(9,7)*+{\bt}'(9,8)*+{\bt}*\frm{-}'(9,9)*+{\bt}
               '(8,9)*+{\bt}*\frm{-}'(7,9)*+{\bt}'(6,9)*+{\bt}
			   '(5,9)*+{\bt}*\frm{-}'(4,9)*+{\bt}
			   '(3,9)*+{\bt}'(2,8)*+{\bt}'(1,7)*+{\bt}*\frm{-}
			   '(0,6)*+{\bt}'(0,5)*+{\bt}*\frm{-}'(0,4)*+{\bt}
		   '(0,3)*+{\bt}'(0,2)*+{\bt}*\frm{-}'(0,1)*+{\bt}'(0,0)},
{(1,1)*+{*}*\frm{-}\PATH~={**\dir{.}}
               '(2,1)*+{*}'(3,1)*+{*}'(4,2)*+{*}
               '(5,3)*+{*}*\frm{-}'(6,4)*+{*}'(7,5)*+{*}
			   '(8,6)*+{*}*\frm{-}'(8,7)*+{*}'(8,8)*+{*}
			   '(7,8)*+{*}'(6,8)*+{*}*\frm{-}'(5,8)*+{*}
               '(4,8)*+{*}'(3,8)*+{*}*\frm{-}'(2,7)*+{*}
			   '(1,6)*+{*}'(1,5)*+{*}
			   '(1,4)*+{*}*\frm{-}'(1,3)*+{*}'(1,2)*+{*}
			   '(1,1)*+{*}*\frm{-}},
{(2,2)*+{\cr}\PATH~={**\dir{.}}
               '(3,2)*+{\cr}*\frm{-}
               '(4,3)*+{\cr}'(5,4)*+{\cr}
			   '(6,5)*+{\cr}*\frm{-}'(7,6)*+{\cr}
			   '(7,7)*+{\cr}*\frm{-}'(6,7)*+{\cr}
               '(5,7)*+{\cr}
			   '(4,7)*+{\cr}*\frm{-}'(3,7)*+{\cr}
			   '(2,6)*+{\cr}*\frm{-}
			   '(2,5)*+{\cr}'(2,4)*+{\cr}
			   '(2,3)*+{\cr}*\frm{-}'(2,2)*+{\cr}},	   
{(3,3)*+{\tm}\PATH~={**\dir{.}}
               '(4,4)*+{\tm}*\frm{-}
               '(5,5)*+{\tm}'(6,6)*+{\tm}
			   '(5,6)*+{\tm}*\frm{-}'(4,6)*+{\tm}
			   '(3,6)*+{\tm}
			   '(3,5)*+{\tm}*\frm{-}'(3,4)*+{\tm}
			   '(3,3)*+{\tm}},	   	
{(4,5)*+{\tm}},
%
{(4,0)*+{\st}\PATH~={**\dir{--}}'(3,0)*+{\bt}},
{(0,7)*+{\st}\PATH~={**\dir{--}}'(0,6)*+{\bt}},
{(4,11)*+{\st}\PATH~={**\dir{--}}'(3,10)'(3,9)*+{\bt}},
{(11,7)*+{\st}\PATH~={**\dir{--}}'(10,6)'(9,6)*+{\bt}},
{(11,11)*+{\st}\PATH~={**\dir{--}}'(11,10)'(10,9)'
               '(9,9)*+{\bt}'(9,10)'(10,11)'(11,11)},	  		   
%
{(0,0)*+{\bt}\PATH~={**\dir{-}}
               '(1,0)*+{\bt}_{\alpha_1}^{1}
			   '(2,1)*+{*}
			   '(2,2)*+{\cr}
			   '(1,2)*+{*}
			   '(0,1)*+{\bt}
			   '(0,0)*+{\bt}_{\alpha_2}^{2}},
\endxy
\bigskip fig. 8
\medskip
The weight diagram $\fwd_{-\kappa\lambda}$ for $\lambda=(1,2)$
 with multiplicities $1,2,3,4$
depicted by $\bullet\,, *\,, \circ\,, $ x,  respectively; the
edges of the elementary hexagons (except the first one) are
omitted. The same picture describes the mapping of
$\fwd_{-\kappa\lambda}$ into the $sl(3)$ weight diagram
$\Gamma_{3\lambda}$ -- the points removed from the latter are
indicated by squares. The stars $\star$ denote  positions of
singular vectors in the corresponding Verma modules.
\bigskip\vfill\eject
\bigskip

\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
%0;<\hrt cm,.5cm>:<-\hrt cm,.5cm>::
{(0,0)*+{\bt}\PATH~={**\dir{.}}'(1,0)*+{\bt}*\frm{-}_{\alpha_1}
			   '(2,1)*+{\bt}'(3,2)*+{\bt}
			   '(4,3)*+{\bt}*\frm{-}'(5,4)*+{\bt}'(6,5)*+{\bt}
			   '(7,6)*+{\bt}*\frm{-}'(8,7)*+{\bt}
			   '(8,8)*+{\bt}*\frm{-}'(7,8)*+{\bt}
               '(6,8)*+{\bt}'(5,8)*+{\bt}*\frm{-}
			   '(4,8)*+{\bt}'(3,8)*+{\bt}
			   '(2,8)*+{\bt}*\frm{-}'(1,8)*+{\bt}
			   '(0,7)*+{\bt}*\frm{-}
			   '(0,6)*+{\bt}'(0,5)*+{\bt}'(0,4)*+{\bt}*\frm{-}
			   '(0,3)*+{\bt}'(0,2)*+{\bt}'(0,1)*+{\bt}*\frm{-}
			   '(0,0)_{\alpha_2}},
{(1,1)*+{*}\PATH~={**\dir{.}}
               '(2,2)*+{*}*\frm{-}'(3,3)*+{*}'(4,4)*+{*}
               '(5,5)*+{*}*\frm{-}'(6,6)*+{*}'(7,7)*+{*}
			   '(6,7)*+{*}*\frm{-}'(5,7)*+{*}'(4,7)*+{*}
			   '(3,7)*+{*}*\frm{-}'(2,7)*+{*}
               '(1,7)*+{*}
			   '(1,6)*+{*}*\frm{-}'(1,5)*+{*}
			   '(1,4)*+{*}'(1,3)*+{*}*\frm{-}'(1,2)*+{*}
			   '(1,1)*+{*}},
{(2,3)*+{*}\PATH~={**\dir{.}}
               '(3,4)*+{*}*\frm{-}'(4,5)*+{*}'(5,6)*+{*}
			   '(4,6)*+{*}*\frm{-}'(3,6)*+{*}
			   '(2,6)*+{*}
			   '(2,5)*+{*}*\frm{-}'(2,4)*+{*}'(2,3)*+{*}},	   
{(3,5)*+{*}},
%
{(2,0)*+{\st}\PATH~={**\dir{--}}'(2,1)*+{*}},
{(0,8)*+{\st}\PATH~={**\dir{--}}'(1,8)*+{*}},
{(2,10)*+{\st}\PATH~={**\dir{--}}'(2,9)'(1,8)*+{}},
{(10,8)*+{\st}\PATH~={**\dir{--}}'(9,8)'(8,7)*+{*}},
{(10,10)*+{\st}\PATH~={**\dir{--}}'(9,9)'(9,8)},			   
%
{(0,0)*+{\bt}\PATH~={**\dir{-}}'(1,1)*+{*}^{0}},
{(2,1)*+{\bt}\PATH~={**\dir{-}}'(1,1)*+{*}^{1}
               '(1,2)*+{*}^{2}'(0,2)*+{\bt}^{0}},
{(2,1)*+{\bt}\PATH~={**\dir{-}}'(3,2)*+{\bt}^{2}
               '(3,3)*+{*}^{1}'(2,3)*+{*}^{2}'(1,2)*+{*}^{1}},
\endxy
\bigskip fig. 9
\medskip
The weight diagram $\fwd_{w_3\cdot(-\kappa\lambda)}$
and its mapping  into the $sl(3)$ weight diagram
$\Gamma_{3\lambda-2\rho}$ for $\lambda=(1,3)$. The multiplicities
$1,2$ are depicted  by $\bullet\,, *\,, $  respectively.
\bigskip

\xy 
0;<\hrt cm,.5cm>:<-\hrt cm,.5cm>::
{(-1,2)\PATH~={**\dir{.}}'(1,0)'(2,-1)},
{(-3,-2)\PATH~={**\dir{.}}'(1,0)'(3,1)},
{(2,2)\PATH~={**\dir{.}}'(1,0)'(0,-2)},
{(0,0)*+{a0}*\frm{o} \PATH ~={**\dir{-}}
                '(1,1)*+{??}*\frm{-}^0},
{(0,0)*+{a0}*\frm{o} \PATH ~={**\dir{-}}
                '(0,-1)*+{??}*\frm{-}^2},
{(0,0)*+{a0}*\frm{o} \PATH ~={**\dir{-}}
                '(-1,0)*+{1a}*\frm{-}_1}
				
\endxy
\bigskip fig. 10
\medskip %\noindent
The fusion $[[1,1]]\otimes[a,0]=[[1,a]]$, (for short $a=p-1$). 
The weights of the shifted diagram ${\cal G}_{[[1,1]]}\circ[a,0]$
outside the admissible alcove are indicated by ??. Each one of
them is of multiplicity one and together cancel the weight [a,0].
\bigskip\bigskip


\hbox{ 
\vbox{
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(-.3,.3)*+{\Lambda^*}},
{(0,0)*+{1}*\frm{o}\PATH ~={**\dir{-}}
            '(1,1)*+{2}*\frm{o}^0
            '(2,1)*+{2}*\frm{o}^1'(2,0)*+{1}*\frm{o}^0
			'(3,0)*+{1}*\frm{o}^2'(4,1)*+{2}*\frm{o}^0
            '(5,1)*+{1}*\frm{o}^1},
%
{(1,1)*+{2}\PATH ~={**\dir{-}}'(1,2)*+{1}*\frm{o}^2
            '(2,3)*+{1}*\frm{o}^1'(3,3)*+{2}*\frm{o}^2
			'(3,2)*+{2}*\frm{o}^1'(4,2)*+{2}*\frm{o}^0
            '(4,1)*+{2}*\frm{o}^2},
%
{(2,1)*+{2}\PATH ~={**\dir{-}}'(3,2)*+{2}^2},
{(3,3)*+{2}\PATH ~={**\dir{-}}'(4,4)*+{2}^0},
%
{(4,2)*+{2}*\frm{o}\PATH ~={**\dir{-}}
              '(5,3)*+{1}*\frm{o}^1'(5,4)*+{1}*\frm{o}^0
			  '(4,4)*+{2}*\frm{o}^1'(4,5)*+{1}*\frm{o}^2},
\endxy} \hskip 2cm
\vbox{
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(0,0)*+{22}*\frm{-}\PATH ~={**\dir{-}}'(1,1)*+{11}*\frm{o}^0
            '(2,1)*+{a1}*\frm{-}^1'(2,0)*+{b0}*\frm{o}^0
			'(3,0)*+{??}*\frm{-}^2'(4,1)*+{??}*\frm{o}^0
            '(5,1)*+{??}*\frm{-}^1},
%
{(1,1)*+{11}\PATH ~={**\dir{-}}'(1,2)*+{1a}*\frm{-}^2
            '(2,3)*+{a1}*\frm{o}^1'(3,3)*+{11}*\frm{-}^2
			'(3,2)*+{1a}*\frm{o}^1'(4,2)*+{??}*\frm{-}^0
            '(4,1)*+{??}*\frm{o}^2},
%
{(2,1)*+{a1}\PATH ~={**\dir{-}}'(3,2)*+{1a}^2},
{(3,3)*+{11}\PATH ~={**\dir{-}}'(4,4)*+{00}^0},
%
{(4,2)*+{??}*\frm{-}\PATH ~={**\dir{-}}
              '(5,3)*+{??}*\frm{o}^1'(5,4)*+{??}*\frm{-}^0
			  '(4,4)*+{00}*\frm{o}^1'(4,5)*+{??}*\frm{-}^2},
{(2,-1)\PATH ~={**\dir{.}}'(5,5)'(1,3)'(-1,2)}
\endxy}} 

\bigskip fig. 11 
\medskip%\noindent
The fusion $[[2,1]]\otimes [0,1] = 
[[2,2]]\oplus [1,1] \oplus [[1,a]] \oplus
[[1,1]] \oplus [a,1]$, \quad $a=p-2$.

\bigskip\bigskip

\vskip 4cm


\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(6.5,5.5)*+{(0,0)}},{(-2.2,.9)*+{(12,0)}},{(1.8,-3.1)*+{(0,12)}},
{(-.2,-.2)*+{\mu}},
{(6,5)*+{\bt}*\frm{-}\PATH ~={**\dir{.}}
          '(4,4)*+{\cr}*\frm{-}'(2,3)*+{\cr}*\frm{-}
		  '(0,2)*+{\bt}*\frm{-}
		  '(-2,1)'(2,-3)'(4,1)*+{\bt}*\frm{-}
		  '(5,3)*+{*}*\frm{-}'(6,5)*+{\bt}*\frm{-}},
%
{(6,5)*+{\bt}*\frm{-}\PATH ~={**\dir{--}}
          '(6,6)*+{\bt}'(5,6)*+{\bt}*\frm{-}'(3,6)
		  '(1,4)*+{\bt}*\frm{-}'(0,3)
		  '(0,2)*+{\bt}*\frm{-}
		  '(0,0)'(2,0)*+{\bt}*\frm{-}'(3,0)
		  '(4,1)*+{\bt}*\frm{-}'(6,3)'(6,5)*+{\bt}*\frm{-}},
{(2,1)*+{*}\PATH ~={**\dir{--}}'(1,1)*+{*}*\frm{-}'(1,2)*+{*}},
{(4,2)*+{*}\PATH ~={**\dir{--}}'(5,3)*+{*}*\frm{-}'(5,4)*+{*}},
{(2,4)*+{*}\PATH ~={**\dir{--}}'(3,5)*+{*}*\frm{-}'(4,5)*+{*}},
{(2,2)*+{\cr}\PATH ~={**\dir{--}}'(2,3)*+{\cr}*\frm{-}'(3,4)*+{\cr}},
{(2,2)*+{\cr}\PATH ~={**\dir{--}}'(3,2)*+{\cr}*\frm{-}'(4,3)*+{\cr}},
{(4,3)*+{\cr}\PATH ~={**\dir{--}}'(4,4)*+{\cr}*\frm{-}'(3,4)*+{\cr}},
% 
{(1,0)*+{\bt}\PATH ~={**\dir{-}}
 '(0,0)*+{\bt}^1'(0,1)*+{\bt}^2},
%
{(1,0)*+{\bt}\PATH ~={**\dir{-}}'(2,1)*+{*}^2},
{(0,1)*+{\bt}\PATH ~={**\dir{-}}'(1,2)*+{*}^1},
%
{(3,0)*+{\bt}\PATH ~={**\dir{-}}
		 '(3,1)*+{*}^2'(2,1)*+{*}^0
		 '(2,2)*+{\cr}^1'(1,2)*+{*}^2
         '(1,3)*+{*}^0'(0,3)*+{\bt}^1},
%
{(3,1)*+{*}\PATH ~={**\dir{-}}'(4,2)*+{*}^1},
{(2,2)*+{\cr}\PATH ~={**\dir{-}}'(3,3)*+{\tm}^0},
{(1,3)*+{*}\PATH ~={**\dir{-}}'(2,4)*+{*}^2},
%
{(5,2)*+{\bt}
		   \PATH ~={**\dir{-}}
		   '(4,2)*+{*}^2'(4,3)*+{\cr}^0
		   '(3,3)*+{\tm}^1'(3,4)*+{\cr}^2
		   '(2,4)*+{*}^0'(2,5)*+{\bt}^1},
%
{(5,2)*+{\bt}\PATH ~={**\dir{-}}'(6,3)*+{\bt}^0},
{(4,3)*+{\cr}\PATH ~={**\dir{-}}'(5,4)*+{*}^2},
{(3,4)*+{\cr}\PATH ~={**\dir{-}}'(4,5)*+{*}^1},
{(2,5)*+{\bt}\PATH ~={**\dir{-}}'(3,6)*+{\bt}^0},
%
{(6,3)*+{\bt}
			  \PATH ~={**\dir{-}}
			  '(6,4)*+{\bt}'(5,4)*+{*}^0
			  '(5,5)*+{*}^1'(4,5)*+{*}^2
			  '(4,6)*+{\bt}^0'(3,6)*+{\bt}^1},
%
{(5,5)*+{*}\PATH ~={**\dir{-}}'(6,6)*+{\bt}^0},
\endxy
\bigskip fig. 12 
\medskip %\noindent
The comparison of the fusion 
 $[1,1]\otimes[1,0]$ and $(3,3)\otimes(3,0)$.
 The convention for multiplicities is as in fig. 8.


\bye


\xy 
0;<\hrt cm,.5cm>:<-\hrt cm,.5cm>::
{(-1,-1)\PATH~={**\dir{.}}'(3,1)},
{(-1,-1)\PATH~={**\dir{.}}'(1,3)},
{(-2,0)\PATH~={**\dir{.}}'(0,-2)},
{(0,0)*+{00}*\frm{o} \PATH ~={**\dir{-}}
                '(1,1)*+{11}*\frm{-}^0},
{(0,0)*+{00}*\frm{o} \PATH ~={**\dir{-}}
                '(0,-1)*+{0p}*\frm{-}^2},
{(0,0)*+{00}*\frm{o} \PATH ~={**\dir{-}}
                '(-1,0)*+{p0}*\frm{-}_1}	
		
\endxy
\bigskip fig. 11
\medskip%\noindent
The fusion of [[1,1]] and [0,0]. The dotted lines 
indicate lines from the dual lattice that are borders of 
alcoves, reflecting in them reproduces the action of KW; 
the weights from the shifted diagram
$\fwd_{[[1,1]]}\circ [0,0]$ (coinsiding in this case with the
unshifted one because $\Lambda'=[0,0]$)
that are inside the dominant
admissible alcove are [0,0] and [[1,1]];
${\cal G}_{[[1,1]]}$ has multiplicities 2 for the central point
and 1 for the rest;
the weight [0,0], which is of
multiplicity 2 is mapped under the KW action to the  weights 
$[[p,0]]$ and $[[0,p]]$
of multiplicity 1 so its contribution cancels
\bigskip

\bye

\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
%0;<\hrt cm,.5cm>:<-\hrt cm,.5cm>::
{(0,0)*+{+}*\frm{o}\PATH~={**\dir{.}}
               '(7,0)*+{-}*\frm{o}'(11,4)*+{+}*\frm{o}
			   '(11,11)*+{-}*\frm{o}'(7,11)*+{+}*\frm{o}
			   '(0,4)*+{-}*\frm{o}'(0,0)*+{+}*\frm{o}},
%
{(3,0)\PATH~={**\dir{-}}'(4,0)^1},
%			   
{(0,0)*+{+}*\frm{o}\PATH~={**\dir{-}}'(1,0)^1'(2,1)^2'(2,2)^1
               '(1,2)^2'(0,1)^1'(0,0)*+{+}*\frm{o}^2},
%			   
{(11,4)*+{+}*\frm{o}\PATH~={**\dir{-}}'(12,4)^1'(13,5)^2'(13,6)^1
               '(12,6)^2'(11,5)^1'(11,4)*+{+}*\frm{o}^2},
%			   
{(7,11)*+{+}*\frm{o}\PATH~={**\dir{-}}'(8,11)^1'(9,12)^2'(9,13)^1
               '(8,13)^2'(7,12)^1'(7,11)*+{+}*\frm{o}^2},	
%
{(6,0)\PATH~={**\dir{-}}'(7,0)*+{-}*\frm{o}^1'(8,1)^2},
{(9,0)\PATH~={**\dir{.}}'(7,0)*+{-}*\frm{o}^{\hat 1}
              '(7,2)^{\hat 0}},
{(9,0)\PATH~={**\dir{-}}'(9,1)^{2}'(8,1)^0'(8,2)^1'
              '(7,2)^{2}},			  
%			  
\endxy
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% probably skip in fianl version so put after \bye
%
\bigskip
\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(0,0)*+{\bt}\PATH ~={**\dir{-}}'(3,0)*+{\cr}^1_{m_1}
                                '(4,1)*+{\bt}^0_{m_2}
                                '(4,4)*+{\cr}^2_{m_1}
				'(3,4)*+{\bt}^1_{m_2}
                                '(0,1)*+{\cr}^0_{m_1}
                                '(0,0)*+{\bt}^2_{m_2}}
\endxy

\bigskip


\bigskip probably these two figures are redundant

\xy 
0;<-\hrt cm,-.5cm>:<\hrt cm,-.5cm>::
{(0,0)*+{\cr}\PATH ~={**\dir{-}}'(3,0)*+{\sharp}^1_{m_1-1}
                                '(4,1)*+{\cr}^1_{m_2-1}
                                '(4,4)*+{\sharp}^0_{m_1-1}
				'(3,4)*+{\cr}^0_{m_2-1}
                                '(0,1)*+{\sharp}^2_{m_1-1}
                                '(0,0)*+{\cr}^2_{m_2-1}}
\endxy
\bigskip
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\bye












